Labor Market Effects of the Venezuelan Refugee Crisis in Brazil

We use administrative panel data on the universe of Brazilian formal workers to investigate the labor market effects of the Venezuelan crisis in Brazil, focusing on the border state of Roraima. The results using difference-in-differences show that the monthly wages of Brazilians in Roraima increased by around 2 percent, which was mostly driven by those working in sectors and occupations with no refugee involvement. The study finds negligible job displacement for Brazilians but finds evidence of native workers moving to occupations without immigrants. We also find that immigrants in the informal market offset the substitution effects in the formal market.

==> Old_Files/did_border.tex <==

\begin{tabular}[t]{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-5}
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Border} \\
\cmidrule(l{3pt}r{3pt}){2-5}
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{Entire Market} & \multicolumn{1}{c}{Retail} & \multicolumn{1}{c}{Retail\textsuperscript{2}} & \multicolumn{1}{c}{No Retail} \\
\cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5}
  & (1) & (2) & (3) & (4)\\
\midrule
Treated & \num{-0.004} & \num{-0.105} & \num{-0.070} & \num{0.119}\\
 & (\num{0.039}) & (\num{0.028}) & (\num{0.022}) & (\num{0.050})\\
\midrule
N & \num{6463} & \num{3412} & \num{3028} & \num{3060}\\
Year fixed effects & X & X & X & X\\
Individual fixed effects & X & X & X & X\\
\bottomrule
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{2} Retail results excluding 2008 and 2009 pre-treatment periods.}\\
\end{tabular}


==> Old_Files/did_capital.tex <==

\begin{tabular}[t]{lccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-6}
\multicolumn{1}{c}{ } & \multicolumn{5}{c}{Capital} \\
\cmidrule(l{3pt}r{3pt}){2-6}
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{Entire Market} & \multicolumn{1}{c}{Retail} & \multicolumn{1}{c}{Construction} & \multicolumn{1}{c}{Restaurants} & \multicolumn{1}{c}{Health} \\
\cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6}
  & (1) & (2) & (3) & (4) & (5)\\
\midrule
Treated & \num{0.040} & \num{0.033} & \num{0.077} & \num{0.016} & \num{0.088}\\
 & (\num{0.010}) & (\num{0.020}) & (\num{0.010}) & (\num{0.009}) & (\num{0.044})\\
\midrule
N & \num{504020} & \num{167168} & \num{34078} & \num{15386} & \num{34740}\\
Year fixed effects & X & X & X & X & X\\
Individual fixed effects & X & X & X & X & X\\
\bottomrule
\multicolumn{6}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\end{tabular}


==> Old_Files/did_capital_hetero_educ.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-7}
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Capital} \\
\cmidrule(l{3pt}r{3pt}){2-7}
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Low Education} & \multicolumn{3}{c}{High Education} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{Entire Market} & \multicolumn{1}{c}{Retail} & \multicolumn{1}{c}{Restaurants} & \multicolumn{1}{c}{Entire Market} & \multicolumn{1}{c}{Retail} & \multicolumn{1}{c}{Restaurants} \\
\cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7}
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treated & \num{0.037} & \num{0.042} & \num{-0.003} & \num{0.024} & \num{0.002} & \num{-0.124}\\
 & (\num{0.010}) & (\num{0.025}) & (\num{0.011}) & (\num{0.024}) & (\num{0.022}) & (\num{0.030})\\
\midrule
N & \num{259857} & \num{99976} & \num{7203} & \num{85300} & \num{8521} & \num{257}\\
Year fixed effects & X & X & X & X & X & X\\
Individual fixed effects & X & X & X & X & X & X\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\end{tabular}


==> Old_Files/did_capital_occup75.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-7}
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Occupations in the Capital} \\
\cmidrule(l{3pt}r{3pt}){2-7}
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{High Immigrant Presence} & \multicolumn{3}{c}{Low Immigrant Presence} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{Construction} & \multicolumn{1}{c}{Retail} & \multicolumn{1}{c}{Restaurants} & \multicolumn{1}{c}{Construction} & \multicolumn{1}{c}{Retail} & \multicolumn{1}{c}{Restaurants} \\
\cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7}
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treated & \num{0.202} & \num{-0.018} & \num{-0.065} & \num{0.075} & \num{0.033} & \num{0.018}\\
 & (\num{0.067}) & (\num{0.035}) & (\num{0.026}) & (\num{0.009}) & (\num{0.020}) & (\num{0.010})\\
\midrule
N & \num{358} & \num{1430} & \num{382} & \num{33723} & \num{165762} & \num{15015}\\
Year fixed effects & X & X & X & X & X & X\\
Individual fixed effects & X & X & X & X & X & X\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\end{tabular}


==> Old_Files/did_placebo.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-7}
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Placebo Borders} \\
\cmidrule(l{3pt}r{3pt}){2-7}
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Rondônia} & \multicolumn{2}{c}{Roraima Interior} & \multicolumn{2}{c}{Acre} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{Entire Market} & \multicolumn{1}{c}{Retail} & \multicolumn{1}{c}{Entire Market} & \multicolumn{1}{c}{Retail} & \multicolumn{1}{c}{Entire Market} & \multicolumn{1}{c}{Retail} \\
\cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4} \cmidrule(l{3pt}r{3pt}){5-5} \cmidrule(l{3pt}r{3pt}){6-6} \cmidrule(l{3pt}r{3pt}){7-7}
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treated & \num{-0.009} & \num{-0.037} & \num{0.030} & \num{0.027} & \num{-0.006} & \num{-0.018}\\
 & (\num{0.031}) & (\num{0.024}) & (\num{0.035}) & (\num{0.023}) & (\num{0.035}) & (\num{0.021})\\
\midrule
N & \num{7720} & \num{3432} & \num{6351} & \num{2855} & \num{7323} & \num{3158}\\
Year fixed effects & X & X & X & X & X & X\\
Individual fixed effects & X & X & X & X & X & X\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\end{tabular}


==> Old_Files/econ_concentration.tex <==

\begin{tabular}[t]{lrrrrrrrr}
\toprule
& \multicolumn{4}{c}{Border} & \multicolumn{4}{c}{Capital}\\
\midrule
& \multicolumn{2}{c}{Other Sectors} & \multicolumn{2}{c}{Retail} &\multicolumn{2}{c}{Other Sectors} & \multicolumn{2}{c}{Retail}\\
 \midrule
& N & Percent & N & Percent & N & Percent & N & Percent\\
\midrule
Brazilian & 50 & \num{96.15} & 70 & \num{81.40} & 26807 & \num{96.98} & 16257 & \num{96.01}\\
Venezuelan & 2 & \num{3.85} & 16 & \num{18.60} & 835 & \num{3.02} & 675 & \num{3.99}\\
\bottomrule
\end{tabular}


==> Old_Files/inputprices.tex <==
In this section, we briefly analyze the construction input price variation happening in Roraima. We used the Civil Construction National Index, provided by the Brazilian Institute of Geography and Statistics. from 2012 to 2017. It measures the construction cost per square meter in local currency. We did not find information on the control states; therefore, our comparison group is the national average prices. Figure \ref{fig:inputprices} was generated by subtracting Roraima's input price from the national average. 

The construction industry in Roraima is traditionally more expensive than Brazil's. However, input prices consistently became closer to the cheaper national average in the post-treatment years. The square meter by 2017 became 25 reais cheaper. 

Assuming Venezuelans in Roraima increased demand for neighborhood expansions in Boa Vista, this scenario implies firm owners increased wages benefited from lower input prices, suggesting a reverse causality between immigration and wages.


\begin{figure}[htb!]
    \centering
    \includegraphics[width =0.8\textwidth]{sections/appendix/figures/inputprice.jpeg}
    \caption{Roraima's input price change relative to the national average.}
    \label{fig:inputprices}
\end{figure}

==> Old_Files/occupation_event_study.tex <==
\begin{figure}[h!]
    \centerline{
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/occupation_figures/Construction - Immigrant Occupation75.jpeg}  
        \caption{Construction - Immigrant Occupation}
        \label{fig:esconstruction-immi}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/occupation_figures/Construction - Non-Immigrant Occupation75.jpeg}
        \caption{Construction - Non-Immigrant Occupation}
        \label{fig:esconstruction-nimmi}
    \end{subfigure}%
    }
        \centerline{
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/occupation_figures/Retail - Immigrant Occupation75.jpeg}
        \caption{Retail - Immigrant Occupation}
        \label{fig:esretail-immi}
    \end{subfigure} %
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/occupation_figures/Retail - Non-Immigrant Occupation75.jpeg}
        \caption{Retail - Non-Immigrant Occupation}
        \label{fig:esretail-nimmi}
    \end{subfigure}%
    }
    \centerline{
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/occupation_figures/Restaurants - Immigrant Occupation75.jpeg}   
        \caption{Restaurants - Immigrant Occupation}
        \label{fig:esresta-immi}
    \end{subfigure}%
        \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/occupation_figures/Restaurants - Non-Immigrant Occupation75.jpeg} 
        \caption{Restaurants - Non-Immigrant Occupation}
        \label{fig:esresta-nimmi}
    \end{subfigure} %
    }
    \caption{Event Studies for Job Occupations in the Capital}
    \label{fig:esoccupation}
 \end{figure}

==> Old_Files/placebo_event_study.tex <==

\begin{figure}[h!]
    \centerline{
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/placebo_figures/borderEntire Market - AC.jpeg}  
        \caption{Entire Market - Acre's Town (Plácido de Castro)}
        \label{fig:esplaceboemac}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/placebo_figures/borderEntire Market - RO.jpeg}  
        \caption{Entire Market - Rondônia's Town (Nova Mamoré)}
        \label{fig:esplaceboemro}
    \end{subfigure}%
    }
        \centerline{
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/placebo_figures/borderEntire Market - RR.jpeg}   
        \caption{Entire Market - Roraima's Town (Caroebe)}
        \label{fig:esplaceboemrr}
    \end{subfigure} %
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/placebo_figures/borderRetail - AC.jpeg}
        \caption{Retail - Acre's Town (Plácido de Castro)}
        \label{fig:esplaceboretailac}
    \end{subfigure}%
    }
    \centerline{
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/placebo_figures/borderRetail - RO.jpeg}   
        \caption{Retail -  Rondônia's Town (Nova Mamoré)}
        \label{fig:esplaceboretailro}
    \end{subfigure}%
        \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/appendix/placebo_figures/borderRetail - RR.jpeg}   
        \caption{Retail - Roraima's Town (Caroebe)}
        \label{fig:esplaceboretailrr}
    \end{subfigure} %
    }
    \caption{Event Studies for Placebo Towns}
    \label{fig:esplacebo}
 \end{figure}

==> Old_Files/structuralmodel.tex <==

%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------

\subsection{Border Town}

We present a structural model for the border town where we compare the market with and without the presence of immigrants. 

\subsubsection{Border Town with a native household only}

\noindent
Consider a local economy composed of workers and firms. There is a representative firm for the informal sector and one for the formal sector. Informal sector differ from formal by not paying taxes when hiring workers. Government collects the tax as a fraction of wage.  We assume same wages for formal and informal, however, differing by the labor tax $\tau$, representing Brazilian labor laws and workers' rights. We assume formal firms can only hire individuals formally. Accordingly, informal firms can only hire informally. Labor is the only requirement for output. Goods in this market produced by formal and informal sector are the same. The formal firm's technology is represented by $\phi$ and the informal firm's by $\psi$.

In this scenario with no refugees, we only observe the representative native household $n$. We normalize the unit of labor to one. The household consumes the good to receive utility and has disutility associated with labor. The government balances its budget by giving back to the household a lump-sum quantity represented by $T$.

%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
\paragraph{The Informal Firm Problem}

The representative informal firm allocates native labor $(H_n^i)$ to maximize its profits given wage $(w)$ and a production function $Y_i$, such that:
 
\begin{align}
    \max_{H_n^i} Y_i - w & H_n^i \\
    & \text{s.t. } Y_i = \psi \log(H_n^i)
\end{align}

where $\psi > 0$. The solution to the profit maximization problem can be expressed as


\begin{equation}
    H_n^{i*} = \frac{\psi}{w} \label{eq:informalsolution}
\end{equation}

and, for optimal output,

\begin{equation}
    Y_i^{*} = \psi \left [\log \left (\frac{\psi}{w} \right ) \right ] 
\end{equation}


%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
\paragraph{The Formal Firm Problem}

The representative formal firm allocates native labor $(H_n^f)$ to maximize its profits given wage $(w)$, tax $(\tau)$ and a production function $Y_f$, such that:
 
\begin{align}
    \max_{H_n^f} Y_f - w (1 + \tau) & H_n^f \\
    & \text{s.t. } Y_f = \phi \log(H_n^f)
\end{align}

where $\phi > 0$. The solution to the profit maximization problem can be expressed as


\begin{equation}
    H_n^{f*} = \frac{\phi}{w ( 1 + \tau)} \label{eq:formalsolution}
\end{equation}

and, for optimal output,

\begin{equation}
    Y_f^{*} = \phi \left [\log \left (\frac{\phi}{w ( 1 + \tau)} \right ) \right ] 
\end{equation}


%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
\paragraph{The Native Household Problem}

Native household consumes good $c$ to maximize its logarithmic utility through labor $L_n$, given wage $(w)$, and government policy $T$:

\begin{align}
    \max_{c, L_n} \nu \log c + (1 - \nu) \log (1 - L_n)& \\
    \text{s.t. } c & = w L_n
\end{align}

where $0 < \nu < 1$ is the native household preference parameter. The optimal level of labor and consumption in this household can be expressed as:

\begin{align}
    L_n^* &= \nu \label{eq:optimallabornative1} \\
    c^* &= w \nu
\end{align}

%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------

\paragraph{Markets Clearing Conditions and Government Budget Balance}

The equilibrium is given by wage $w$ such that: 

\begin{align}
    Y_i + Y_f &= c \\ 
    H_n^i + H_n^f &= L_n \\ \label{lmcc}
    w \tau &= T
\end{align}

where the first equation represents the goods market, the second equation represents the labor market and the third equation balances the government budget.

%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
\paragraph{Solving for Wages}

We start by combining the labor market's clearing condition (equation \ref{lmcc}) with the firms' optimal allocation (equations \ref{eq:informalsolution} and \ref{eq:formalsolution}) and the optimal quantity of labor (equation \ref{eq:optimallabornative1}).

\begin{align}
    \frac{\phi}{w ( 1 + \tau)} + \frac{\psi}{w} &= \nu
\end{align}

Rearranging, we finally have:

\begin{align}
    w^*_1 = \frac{\phi}{\nu ( 1 + \tau)} + \frac{\psi}{\nu} \label{eq:bordernativeonlysol}
\end{align}

the intuition behind the solution is the relationship between the household preference and optimal wage. Higher preference parameter implies less disutility coming from labor and consequentially lowering wages.

Equation \ref{eq:bordernativeonlysol} can be interpreted as the classic downward slope demand curve. When native labor supply increases, wage decreases. Also, it is noteworthy the relationship between formal technology and government policy. Roraima is one of the poorest and rural regions of Brazil, where a high informality is observed. If we allow $\phi$ and $\psi$ to have the same value in the model, labor supply in the informal sector becomes much higher depending on the burden created by Brazilian government regulations.


%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
\subsubsection{Adding the immigrant household in the border town economy}

We introduce a second household in our model, $r$, representing the new immigrant population. Accordingly, the immigrant household trades $L_r$ units of labor to receive wage, but must face a penalty $\delta$ associated with immigration challenges. They can work both in formal and informal sector. Brazilian and Venezuelan labor is considered excludable and rivalrous (if the formal sector hires a Venezuelan, it cannot hire a Brazilian to occupy the same position, neither can the informal sector hire the same Venezuelan). However, Venezuelans does not perform as the Brazilians in the production function. The government, as before, taxes labor through the firm and redistribute to the worker as a lump-sum transfer in their budget constraint.

%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------

\paragraph{The Informal Firm Problem with Immigrant Labor Supply}

The representative informal firm allocates native and refugee labor $(H_n^i, H_r^i)$ to maximize its profits given wage $(w)$ and a production function $Y_i$, such that:
 
\begin{align}
    \max_{H_n^i,  H_r^i} Y_i - w & ( H_n^i + \delta H_r^i) \\
    & \text{s.t. } Y_i = \psi \left [ \log(H_n^i + \delta H_r^i) \right ]
\end{align}

where $\psi > 0$ and $0 < \delta < 1$ represents the penalty refugees must pay (such as language barrier, bureaucracy, cost of entry, and prejudice). The solution to the profit maximization problem becomes:


\begin{align}
   H_n^{i*}  + \delta H_r^{i*} &= \frac{\psi}{w} \label{eq:ref_informalsolution}
\end{align}

and, for optimal output,

\begin{equation}
    Y_i^{*} = \psi \left [\log \left (\frac{\psi}{w} \right ) \right ] 
\end{equation}



%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------

\paragraph{The Formal Firm Problem with Immigrant Labor Supply}

The representative formal firm allocates native and refugee labor $(H_n^f, H_r^f)$ to maximize its profits given wage $(w)$, tax $\tau$ and a production function $Y_f$, such that:
 
\begin{align}
    \max_{H_n^f, H_r^f} Y_f - (1 + \tau)( w  & H_n^f + \delta w H_r^f )\\
    & \text{s.t. } Y_f = \phi \left [ \log(H_n^f + \delta H_r^f) \right ]
\end{align}

where $\psi > 0$. The solution to the profit maximization problem can be expressed as


\begin{align}
    H_n^{f*} + \delta H_r^{f*} &= \frac{\phi}{w (1 + \tau)} \label{eq:ref_formalsolution}
\end{align}


and, for optimal output,

\begin{equation}
    Y_i^{*} = \phi \left [\log \left (\frac{\phi}{w ( 1 + \tau)} \right ) \right ] \label{eq:optimalformalo2}
\end{equation}


%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
\paragraph{The Native Household Problem}

Native household consumes $c_n$ to maximize its logarithmic utility through labor $L_n$, given wage $(w)$, and government policy $T_n$:

\begin{align}
    \max_{c_n, L_n} \nu \log c_n + (1 - \nu) \log(1 -  L_n)& \\
    \text{s.t. } c_n & = w L_n
\end{align}

where $0 < \nu < 1$ is the native household preference parameter. The optimal level of labor and consumption in this household can be expressed as:

\begin{align}
    L_n^* &= \nu \label{eq:optimallabornative2} \\
    c_n^* &= w \nu \label{eq:optimalconsunative2}
\end{align}

%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------
\paragraph{The Refugee Household Problem}

Refugee household consumes good $c_r$ to maximize its logarithmic utility through labor $L_r$, given wage $(w)$:

\begin{align}
    \max_{c_r, L_n} \rho \log c_r + (1 - \rho) \log(1 -  L_r) & \\
    \text{s.t. } c_r & = \delta w L_r
\end{align}

where $0 < \nu < 1$ is the native household preference parameter. The optimal level of labor and consumption in this household can be expressed as:

\begin{align}
    L_r^* &= \rho \label{eq:optimallaborrefugee2} \\
    c_r^* &= \delta w \rho
\end{align}

%--------------------------------------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------

\paragraph{Markets Clearing Conditions}

The equilibrium is given by wage $w$ such that: 

\begin{align}
    Y_i + Y_f &= c_n + c_r \\ 
    H_n^i + H_n^f &= L_n \label{lmcc_ref1}\\
    H_r^i + H_r^f &= L_r \label{lmcc_ref1}
\end{align}


\begin{equation}
    H_n^{i*}  + \delta H_r^{i*} + H_n^{f*} + \delta H_r^{f*} = \frac{\phi}{w (1 + \tau)} + \frac{\psi}{w} \label{eq:ref_formalsolution}
\end{equation}


\begin{align}
    \delta \rho + \nu &=  \frac{\phi}{w (1 + \tau)} + \frac{\psi}{w}\\
    \frac{\delta \rho}{\nu} + 1 &= \frac{\phi}{\nu w (1 + \tau)} + \frac{\psi}{\nu w}\\
    w \left (\frac{\delta \rho}{\nu} + 1 \right )&= \frac{\phi}{\nu (1 + \tau)} + \frac{\psi}{\nu} \\
    w_2^* &= \left  (\frac{\nu}{\delta \rho + \nu} \right ) w_1^*
\end{align}




%--------------------------------------------------------------------------------------------------------------------

==> Old_Files/summary_combined.tex <==

\begin{tabular}[t]{llrrrrrr}
\toprule
  &    & Brazilians & & Venezuelans  & &  & \\
\midrule
\midrule
  &    & Mean & Std. Dev. &  Mean & Std. Dev. & Diff. in Means & Std. Error\\
\midrule
Age &  & 36.2 & 10.0 & 30.5 & 8.5 & -5.6 & 0.2\\
Wage &  & 2247.9 & 3158.7 & 1164.6 & 366.5 & -1083.3 & 17.9\\
\midrule
\midrule
 &  & N & Pct. & N & Pct. &  & \\
\midrule
Municipality & Border & 120 & 0.3 & 18 & 1.2 &  & \\
 & Capital & 43064 & 99.7 & 1510 & 98.8 &  & \\
\hdashline
Sector & Other Sectors & 26857 & 62.2 & 837 & 54.8 &  & \\
 & Retail & 16327 & 37.8 & 691 & 45.2 &  & \\
\hdashline
Race & White & 6862 & 15.9 & 94 & 6.2 &  & \\
 & Black & 860 & 2.0 & 15 & 1.0 &  & \\
 & Indigenous & 200 & 0.5 & 2 & 0.1 &  & \\
 & Mixed & 32419 & 75.1 & 915 & 59.9 &  & \\
 & Other or Not Declared & 2843 & 6.6 & 502 & 32.9 &  & \\
 \hdashline
Sex & Female & 17378 & 40.2 & 412 & 27.0 &  & \\
 & Male & 25806 & 59.8 & 1116 & 73.0 &  & \\
\hdashline
Education & No High School & 7400 & 17.1 & 232 & 15.2 &  & \\
 & High School & 29143 & 67.5 & 1128 & 73.8 &  & \\
 & College & 6641 & 15.4 & 168 & 11.0 &  & \\
 \midrule
 \midrule
 Total & &  43 184 & & 1528 & & & \\
\bottomrule
\end{tabular}


==> sections/conclusion.tex <==
In this paper, we conducted a comprehensive analysis of the labor market impacts of the Venezuelan crisis in Brazil, focusing on the state of Roraima, where the crisis had a direct impact. The state's geographical isolation helps us use the immigration shock as a natural experiment, allowing us to gauge the effects on the local labor market. Using a difference-in-differences model, we explored the potential differences in effects based on market diversity in terms of the economic sector and worker occupation.

Our findings revealed that the average monthly wages in Roraima increased by approximately 3 percent in the early stages of the crisis. By analyzing the presence of Venezuelan formal workers by firm's economic sectors and occupation type, we found that Brazilians involved in economic sectors and occupations with a high penetration of Venezuelans had no significant effects on their wages, while the overall wage effect was positive that was driven by those involved in economic sectors and occupations with little to no involvement of Venezuelan immigrants. Using survey data, our analysis of the informal labor market revealed that these workers experienced a significant wage drop. From this, we can conclude that immigrants in the informal labor market acted as complements to the formal labor market, allowing the overall wage to increase and offsetting any substitution effect of foreign workers in the formal labor market.

Our analysis of job displacement and occupation changes further supports these findings. We observed no significant changes in formal employment displacement of Brazilians in Roraima but did find evidence of them moving from high-immigrant occupations to low-immigrant occupations in the post-treatment years. Additionally, we found no effect on the wages in the border municipality, where the economy is less diverse and more than 90 percent of the occupations are manual.

In summary, our study emphasized the need to consider the various factors that can influence the impacts of refugees on the labor market. While our research suggested that refugees can bring benefits, it also highlighted the potential drawbacks of large-scale immigration in regions with a significant informal economy. Moving forward, policymakers should prioritize policies that improve the welfare of refugees and promote their active participation in the economy while also being mindful of the potential negative effects on those working informally. Future research should further explore the impacts of the population boom in Roraima, including improving the understanding of the effects on consumption. It should also seek to untangle the complex situation in Roraima that arose after 2017.

==> sections/data/data.tex <==

%--------------


==> sections/data/summarystatistics.tex <==
An advantage of our data over the Continuous National Household Sample Survey (PNAD-C) household survey used in past studies is the ability to observe the individual's nationality, allowing us to differentiate our sample between Brazilians and Venezuelans. The presence of refugees in our data means they are potential substitutes for natives in the formal market. One mechanism driving the substitution is the education level of the immigrant. If immigrants are willing to accept lower wages and have a clear education profile, for instance, the majority having a high-school diploma, we could see Venezuelans replacing similar higher-paid Brazilians. For this reason, we reserve this subsection to present the demographic characteristics of treated natives and immigrants in our data for 2017, the year with the most significant immigrant presence.

Table \ref{Tab:summary_capital} compares natives and immigrants in the state capital. Wages are reported in local currency (2017's Brazilian real). In 2017, the national minimum wage was around one thousand Brazilian reais. Brazilians in the state capital earned, on average, roughly twice this value, with Venezuelans earning roughly half of their native peers. Brazilians and Venezuelans are at comparable ages in the formal market, around 30 and 34 years, respectively. Venezuelans in the capital are generally male, of mixed race, and with a high-school diploma. None of these qualities seem too far from Roraima's Brazilian citizens' profile. Comparing both sample sizes and the education level distribution, we can conclude that if any substitution effect occurs in Roraima due to immigration, we should expect that the most affected group is the native with completed high school or in related jobs. 

%-------------
\begin{table}[htb!]
\vspace{1cm}
  \centering
 \caption{Summary statistics of Brazilians and Venezuelans in the capital (2017)}
    \label{Tab:summary_capital}
    \resizebox{0.66\textwidth}{!}{\input{sections/data/tables/summary_capital}}
\end{table}
%-------------

The other area in Roraima affected by the immigrants is the border municipality of Pacairama. Table \ref{Tab:summary_border} presents Pacaraima's native-immigrant comparison. Its sample is considerably smaller than the capital, with only 135 natives and 13 immigrants present in 2017. However, the ratio of Venezuelans is higher than in the capital, with 8.7 percent of the formal workers comprised of Venezuelans compared to 2 percent in the capital municipality. It is also worth noting that Venezuelans in the capital and the border are not particularly different, with the majority possessing a high-school diploma.

%-------------
\begin{table}[htb!]
\vspace{1cm}
  \centering
 \caption{Summary statistics of Brazilians and Venezuelans in the border municipality (2017)}
    \label{Tab:summary_border}
    \resizebox{0.66\textwidth}{!}{\input{sections/data/tables/summary_border}}
\end{table}
%-------------

Another noteworthy particularity of Pacaraima is that its residents earn much less than their capital's counterpart on average almost at the same level as the immigrant. This suggests that Brazilian and Venezuelan occupations are highly heterogeneous conditional on their location. In the capital, there is a larger array of job types, allowing natives to seek jobs with less intensive manual labor, or ``low-skilled jobs''. At the border, job occupation is ``flatter'', making both nationalities compete more directly, given Venezuelans generally occupy jobs not requiring college degrees. We provide more details regarding occupations in Roraima in our mechanism section.  




==> sections/data/tables/summary_border.tex <==

\begin{tabular}[t]{lllrr}
\toprule
  &    &     & Brazilian & Venezuelan\\
\midrule
  Average Monthly Wage&  & Mean & \num{1419.65} & \num{1131.68}\\
  \midrule
 Age & & Mean & \num{33.42} & \num{25.85}\\
 \midrule
Race & White & \% & \num{19.26} & \num{0.00}\\
 & Black & \% & \num{0.74} & \num{0.00}\\
 & Indigenous & \% & \num{0.74} & \num{0.00}\\
 & Mixed & \% & \num{74.81} & \num{84.62}\\
 & Not Declared & \% & \num{4.44} & \num{15.38}\\
  \midrule
Sex & Female & \% & \num{44.44} & \num{30.77}\\
 & Male & \% & \num{55.56} & \num{69.23}\\
  \midrule
Education & No High School & \% & \num{8.15} & \num{0.00}\\
 & High School & \% & \num{82.96} & \num{92.31}\\
 & College & \% & \num{8.89} & \num{7.69}\\
 \midrule
N  & & & \num{135} & \num{13}\\
\bottomrule
\end{tabular}


==> sections/data/tables/summary_capital.tex <==

\begin{tabular}[t]{lllrr}
\toprule
  &    &     & Brazilian & Venezuelan\\
\midrule
Average Monthly Wage & & Mean & \num{2200.98} & \num{1184.69}\\
\midrule
Age &  & Mean & \num{34.32} & \num{30.57}\\
\midrule
Race & White & \% & \num{14.75} & \num{5.10}\\
 & Black & \% & \num{1.81} & \num{1.38}\\
 & Indigenous & \% & \num{0.48} & \num{0.21}\\
 & Mixed & \% & \num{69.93} & \num{58.77}\\
 & Not Declared & \% & \num{13.03} & \num{34.54}\\
 \midrule
Sex & Female & \% & \num{43.55} & \num{26.57}\\
 & Male & \% & \num{56.45} & \num{73.43}\\
 \midrule
Education & No High School & \% & \num{18.78} & \num{15.94}\\
 & High School & \% & \num{65.59} & \num{72.90}\\
 & College & \% & \num{15.63} & \num{11.16}\\
  \midrule
N & & & \num{45275} & \num{941}\\
\bottomrule
\end{tabular}


==> sections/intro/introduction.tex <==
The humanitarian crisis in Venezuela, driven by the regime of Nicolás Maduro, has caused more than five million Venezuelans to flee their country. By the time this paper was written, Brazil received approximately a quarter million refugees \citep{unhcr_venezuela_2022}, crossing the border every year at an increasing rate. Most of the refugees from Venezuela entered Brazil by land, using the only highway that connects the two countries through the Brazilian state of Roraima.

There is a scarcity of research on the potential dynamics between formal and informal labor markets in the face of an immigration shock, particularly in the context of developing countries. Our study seeks to investigate the causal relationship between the refugee crisis and the labor market in Roraima, a Brazilian state directly impacted by the crisis. Roraima's geographic isolation from the rest of Brazil presents a unique natural experiment to explore this issue. By employing a comprehensive administrative dataset of formal Brazilian workers and utilizing a difference-in-differences approach, we analyze Roraima in comparison to similar states unaffected by the crisis. This comparative method allows us to investigate the potential effects on wages and job displacement while capitalizing on the sociodemographic parallels among the populations within the region.

Our main findings show a small but significant positive impact on the average monthly wages of Brazilians living in the treated state. This was primarily driven by a positive wage change for those working in economic sectors and occupations with little involvement of refugees. Those involved in sectors and occupations with a higher share of refugees did not experience any significant change in wages following the crisis. We also find that the crisis did not dismiss Brazilians from their jobs and find evidence of them moving to occupations with fewer immigrant shares. These findings suggest that when not directly competing with native workers, Venezuelans acted as complements, increasing formal labor market wages.

Survey data also reveals adverse effects on wages in the informal labor market. Based on the number of refugee status requests and the observations in our administrative data, we believe that many immigrants sought employment and may have found work informally, which, although complemented the formal labor market, also negatively impacted the native wages of individuals in the informal labor market. This explains why we do not see any adverse effects in the formal labor market. For example, when we focus on the border municipality where many jobs are heavily based on manual tasks and where there is a heavy presence of informal workers, we observe close to zero effects on wages, suggesting that any downward pressure on wages caused by Venezuelan immigrants in the formal labor market is offset by the presence of immigrants outside of it.

We contribute to the literature by providing further evidence of the effects of immigration conditional on market characteristics, specifically, the diverse effects by occupation type, economic sector, and formality in the developing region context. The deviation from the canonical approach to immigration is in line with \cite{peri_task_2009, manacorda_impact_2012, dustmann_effect_2013, foged_immigrants_2016}, who argue that immigrants are imperfect substitutes to natives, have a potentially different skill set, and specializes with positive efficiency.

Refugees\footnote{In the period of our study, the Venezuelans displaced by the crisis were virtually the only non-Brazilian population in the state of Roraima. Therefore, specifically for this paper, we refer to Venezuelan refugees as immigrants or foreigners, interchangeably.} comprise a distinct subset of immigrants due to their more vulnerable societal position. Unlike other immigrant groups, their displacement is mainly involuntary. In most cases, host countries for economic immigrants are high-income nations, whereas less-developed countries host most of the world's refugees \citep{cortes_are_2004, taylor_economic_2016}, primarily neighboring countries. For instance, \cite{card_impact_1990, peri_labor_2019, clemens_labor_2019} found no significant results on the 1980 Mariel Boatlift from Cuba on Miami's wages, with \cite{borjas_wage_2017} arguing immigrants may act as substitutes when conditional on education level.

A nascent literature explores this question from the developing country perspective \citep{maystadt_winners_2014, ruiz_labour_2016, taylor_economic_2016, alix-garcia_refugee_2018}. However, due to data limitations or the economic context of the host regions, these studies have primarily overlooked the impact on the formal labor market sector, an aspect our paper aims to address.

The more recent literature on the economic effects of refugees revolves around the Syrian and Venezuelan crises, which shows no evidence of the adverse labor market impacts in neighboring countries' labor markets \citep{fallah_impact_2019, bahar_fools_2018}. Specifically, \cite{bahar_give_2021} studies the labor market impacts of an extensive migratory amnesty program that granted work permits to nearly half a million undocumented Venezuelan migrants in Colombia in 2018. Their analysis indicates no significant impact of the program on hours worked, wages, or labor force participation of Colombian workers. Nonetheless, they study only the immediate effects of the amnesty program without considering its potential dynamic effects in the years following the treatment.

\cite{ryu_refugee_2022} addresses this question from the Brazilian perspective. Using a national quarterly household survey, they use a synthetic control method to study the labor market impacts of Brazilian refugees in Roraima, the affected state, finding that the crisis lowered labor force participation and employment rate in Roraima and did not find any effects on wages. However, the dataset did not distinguish Brazilians and Venezuelans, which could underestimate the effects of refugees. We, therefore, build upon these studies by employing a rigorous administrative panel dataset of the universe of formal workers in Brazil that allows us to distinguish the nationality of individuals and which enables us to use individual-level fixed effects to control for time-invariant unobservables. Our approach also allows us to test for dynamic effects for several years following the start of the crisis.

We organize the remainder of the paper as follows. Section \ref{sec:background} provides the background. Section \ref{sec:data} describes the data. Section \ref{sec:methods} discusses our identification strategy and empirical methodology. Section \ref{sec:results} presents the main results of our model. Section \ref{sec:robustnesschecks} explains our robustness checks based on event studies and placebo tests. Section \ref{sec:mechanisms} discusses the mechanisms through the immigrants are affecting native wages. Section \ref{sec:conclusion} concludes.


==> sections/mechanisms/consumption_analysis.tex <==
Finally, we examine the impacts of the refugee crisis on labor demand in Roraima. We follow \cite{bodvarsson_measuring_2008} by considering the fact that immigrants not only supply labor but also demand goods and services in the local economy, which can create employment opportunities and increase the earnings of the host population. To examine whether the refugee crisis increased consumption in Roraima, we use data from the IBGE's Commerce Monthly Survey (PMC in Portuguese). PMC measures sales volumes in the formal labor market using the state's January 2014 sales as a reference point. For example, if Roraima showed 115 points in formal sales in March 2015, sales would have increased by 15 percent since January 2014.

We use three different regression models to measure the refugee crisis's effects on consumption. First, we use an ordinary least squares (OLS) model that excludes control states and fixed effects, to directly examine the relationship between the number of Venezuelans in Roraima (as measured by RAIS) and the local sales volume. Second, we add back the control states and use a two-way fixed effect regression with a continuous treatment variable represented by the number of immigrants. Finally, we use the same regression model as before but with a binary treatment variable. In all cases, we use RAIS data to measure the monthly number of Venezuelans as a proxy for the total immigrant population in Roraima.

Equation \ref{eq:consumption_eqn} represents the models:

\begin{equation} \label{eq:consumption_eqn}
    log(CI_{st}) = \beta D_{st} + \theta_s + \alpha_t + \epsilon_{ist}
\end{equation}

where the outcome variable, $log(CI_{st})$ is the log of monthly state-level retail sales volume index, $\theta_s$ is the state fixed effects, and $\alpha_t$ is the month fixed effects. $D_{st}$ represents the net amount of Venezuelans by the hundreds for each month extracted from RAIS if the model employed is OLS or the Continuous Treatment model. For the binary treatment, it becomes an indicator function valuing 1 after 2013. We exclude the fixed effects and the sample from the control states in our OLS measurement.

\begin{table}[htb]
    \vspace{1cm}
    \centering 
    \caption{Consumption Analysis}
    \label{tab:consumption}
    \resizebox{.66\textwidth}{!}{\input{sections/mechanisms/tables/sales_results.tex}}
\end{table}

Table \ref{tab:consumption} shows that an increase of one hundred Venezuelans in RAIS leads to a 3 percent increase in sales in our OLS analysis, the same for the continuous treatment model. Our binary treatment study yielded a 30 percent increase in sales after the Venezuelan humanitarian crisis if we compare Roraima with Acre and Amapá.

There were 1,500 Venezuelans in the formal labor market in Roraima in 2017. Therefore, based on our calculations using the estimates from the continuous treatment model, we find that the additional 1,500 Venezuelans in RAIS in 2017, likely resulted in a 45 percent increase in sales. This estimate is within the confidence interval derived from our binary treatment analysis. It is important to note that the number of Venezuelans in RAIS is a proxy for the entire Venezuelan refugee population in Roraima since not all were involved in the formal economic sector and that the number of Venezuelans in the formal labor market is positively proportional to the total number of Venezuelans in Roraima.

The increase in sales is consistent across all of our models. In summary, Table \ref{tab:consumption} suggests that labor demand increased during the crisis, at least in the formal labor market, possibly contributing to the wage increase.


==> sections/mechanisms/formalsector_analysis.tex <==
Now that we have established that there is no evidence of job displacement among Brazilians due to the crisis, we explore the mechanisms that lead to wage increases in the formal labor market. Economists often consider that immigration is not evenly balanced across groups of workers. For example, if high school graduates are the majority of immigrants, they potentially compete with native high school graduates, but not necessarily with individuals holding a college degree \citep{card_is_2005, card_immigration_2009, borjas_wage_2017, llull_immigration_2018}. Another dimension is occupation, wherein immigrants tend to occupy manual-intensive or low-skilled jobs \citep{foged_immigrants_2016}, which could increase the efficiency of the market and allow the overall average wages to grow.

%-----------------------------------------------------------------------------------------------------------------------------
\subsubsection{Effects by Education Level}
\input{sections/mechanisms/subsubsections/education.tex}

%-----------------------------------------------------------------------------------------------------------------------------
\subsubsection{Effects by Economic Sector and Occupation}
\input{sections/mechanisms/subsubsections/occupation.tex}

%-----------------------------------------------------------------------------------------------------------------------------
\subsubsection{Mobility across Occupations}
\input{sections/mechanisms/subsubsections/occupation_mover.tex}


==> sections/mechanisms/informal_analysis.tex <==
Our analysis so far has demonstrated that the overall market experienced positive effects during the immigration crisis. Additionally, we found that only individuals not directly involved in occupations or economic sectors with sizeable Venezuelan presence saw a wage increase in formal employment. However, if immigrants are complementary (substitute) to workers in non-manual (manual) occupations, we expect the Venezuelan immigrants in RAIS to cause wages to decline in manual labor occupations where they are concentrated. Despite this expectation, we did not observe any negative effects in these positions.

One way to interpret these results is to consider the role of Venezuelan immigrants who are not part of the formal market. We showed that many Venezuelan immigrants in the region had sought refugee status, but only a small percentage have entered the formal market. This suggests that many of them are working informally or in seek of employment. Informal workers tend to have lower levels of education and specialize in manual tasks, while those in the formal labor market often hold cognitive or technical jobs, with some overlap. 

In Roraima, about 45 percent of the workforce is involved in the informal labor market. To analyze whether there are any negative impacts on wages in the informal labor market, we use data from the PNAD-C from 2012-17. PNAD-C is a representative household survey conducted by the Brazilian Institute of Geography and Statistics (IBGE) every trimester that includes socio-economic and demographic information, such as household composition, education, employment, income, migration, fertility, etc. However, a major limitation of this data is that, unlike RAIS, it does not include information on the respondents' nationality, municipality, or personal identification. This means we cannot directly analyze the impacts on Brazilian citizens or use individual fixed effects to control for time-invariant individual characteristics. As a result, the inclusion of Venezuelan immigrants in our wage regression sample overestimates the magnitude of coefficients.

We use equation \ref{eq:pnad_did} which is identical to equation \ref{eq:wagesdid} except that we use the state fixed effects term, $\theta_s$, instead of individual fixed effects, due to PNAD-C being a repeated cross-sectional dataset at the state level.

\begin{equation} \label{eq:pnad_did}
    y_{ist} = \beta D_{st} + f(X_{it}) + \theta_s + \alpha_t + \epsilon_{ist}
\end{equation}

Table \ref{tab:informal_analysis} shows the results of this analysis using equation \ref{eq:pnad_did}. Those in the informal labor market in the Roraima experienced around a 24 percent decrease in wages compared to the control states. This is, however, a lower bound of the effect given the presence of Venezuelans in the data sample.

\begin{table}[htb]
    \vspace{1cm}
 \centering
 \caption{Effects in the Informal Labor Market}
    \label{tab:informal_analysis}
    \input{sections/mechanisms/tables/informal_results.tex}
\end{table}

These findings suggest that native workers in the formal labor market may have benefited from the presence of immigrant workers in informal jobs by increasing their efficiency. We observed negative effects on wages in the informal labor market, but no negative effects for jobs with a significant Venezuelan presence in RAIS together with positive effects in jobs not related to immigration, confirming that the refugees in informal employment may have depressed wages locally, but offset the substitution effect of formally hired immigrants.% We provide a theoretical framework in the appendix to help explain these results in more detail.

==> sections/mechanisms/mechanisms.tex <==
There are three main channels through which immigration could positively affect the formal labor market wages in Roraima. We list them below sorted by the decreasing strength of our measurement conditional on data quality.
\begin{enumerate}
    \item Immigrants in the formal labor market can affect wages by substituting for certain native jobs and complimenting others. However, the complementary effects are stronger than the substitution effects, resulting in an overall positive change.
    \item Immigrants working informally outside the formal market can increase wages through complementarity.
    \item The presence of the immigrant population as a whole can increase native wages by boosting consumption and labor demand.
\end{enumerate}


\subsection{Job Displacement of Native Workers}
\input{sections/mechanisms/unemployment.tex}

\subsection{Mechanisms in the Formal Labor Market}
\input{sections/mechanisms/formalsector_analysis.tex}

\subsection{Effects in the Informal Labor Market}
\input{sections/mechanisms/informal_analysis.tex}

\subsection{Consumption Effects of Refugees}
\input{sections/mechanisms/consumption_analysis.tex}


==> sections/mechanisms/subsubsections/education.tex <==
Our sample does not have a meaningful contrast in education among natives and immigrants. Still, there is no employment displacement although the immigrant wages are significantly lower. Hence, the question of whether there are any meaningful wage substitution effects through education cohorts arises.

We focus on the state capital sample, dividing it into three education cohorts: college-educated, high-school-educated, and low-education, or those with less than high school education. We again employ the model represented in Equation \ref{eq:wagesdid}. Results are shown in Table \ref{tab:educationresults}.

\begin{table}[htb]
    \vspace{1cm}
    \caption{Education Results}
    \label{tab:educationresults}
    \resizebox{\textwidth}{!}{\input{sections/mechanisms/tables/educationresults.tex}}
\end{table}

Columns (1), (2), and (3) show the results for the low education sample, Columns (4), (5), and (6) represent the high school sample, while Columns (7), (8), and (9), represent the college-educated sample. Results for low education and college-degree natives, the two groups underrepresented by Venezuelans, reveal that after the crisis, they experienced on average 3 percent increase in wages. If we balance the panel data by only keeping individuals with counterfactuals, results for low-education individuals increases to 5 percent.

Results for high-school individuals are slightly lower in magnitude and less precise, at around 2 percent. This education level corresponds to 72 percent of all Venezuelans in Roraima's RAIS. We could assume these weaker results are due to the Venezuelan presence, however, we still observe significant positive results, implying that if substitution effects exist at all, they are being offset by other effects. We are aligned with \cite{card_impact_1990} and \cite{clemens_labor_2019} where we do not see any negative effects for low-education or high-school individuals in the labor market. Moreover, the wage increase in the aggregate market suggests immigrants acted as a complementary workforce elsewhere, not necessarily inside the formal labor market.


==> sections/mechanisms/subsubsections/occupation.tex <==
A direct approach to test if immigrants inside the formal labor market had effects on wages, independent of education cohorts, is to explore the channels of occupation and related economic sectors.

Our first analysis consists of creating a variable measuring the Venezuelan-Brazilian ratio in a given set of firms based on economic sectors. We then sample the native workers based on the percentile of this ratio. We consider economic sectors with high immigrant concentration with a ratio above the 75th percentile, and, likewise, under the 25th percentile for low concentration.

At first glance, immigrants observed in RAIS allocated themselves to firms requiring more manual labor. These areas were, among others, retail sales, restaurants, construction, agriculture, transformation, copiers, and veterinary. The ones not related were, among others, finance, insurance, telecommunication, research, pharmaceutics, and entertainment. The generated samples' regression results are shown in Table \ref{tab:activity_results}.

\begin{table}[htb]
    \vspace{1cm}
    \centering
    \begin{threeparttable}
        \caption{Effects by Firm Economic Sector Conditional on Immigrant Presence}  \label{tab:activity_results}
        \input{sections/mechanisms/tables/activity_results.tex}
    \end{threeparttable}
  \end{table}

Columns (1), (2), and (3) present results for the 75th percentile and above. They were close to zero for our unbalanced data and at 1.1 percent when using the balanced version, failing to reject the null hypothesis at a 5 percent confidence interval. Contrarily, for economic sectors falling in the lower 25th percentile in terms of immigrant presence showed, on average, a 6 percent increase in wages after the Venezuelan crisis.

These measurements suggest heterogeneity across economic sectors when we condition on immigrant presence. Another direct approach to investigate the role of Venezuelans in the formal labor market is to sample based on workers' occupation instead of firm's economic sector, using the RAIS variable that describes their responsibilities at a job. We used the same percentile procedure as before with a slight variation. We first separated occupations where we did not observe foreigners in our data. Then we run our regressions on three samples. The first sample corresponds to individuals in the immigrant presence ratio at the 75th percentile and above, conditional on occupations where we observe immigrants. The second sample is any occupation we observe at least one Venezuelan working. Finally, the third sample is all individuals without immigrants in their occupations.

We also use the description of these occupations to assign if they are related to manual labor. For occupations where no immigrants were observed, 51.5 percent can be considered manual. When we count the immigrant occupations, this percentage jumps to 81.8 percent. The 75th percentile cohort yields 90 percent of manual labor. Venezuelans in our data were generally cashiers, technicians, bakers, car mechanics, waiters, receptionists, painters, and others. Although we observe similar jobs in non-immigrant occupations, there was a considerable number of directors, managers, engineers, doctors, professors, etc.

The immigration wage effect regressions based on these samples are shown in Table \ref{tab:occupation_results}.

\begin{table}[htb]
    \vspace{1cm}
        \centering
        \begin{threeparttable}
            \caption{Effects by Worker Occupation Conditional on Immigrant Presence} \label{tab:occupation_results}
            \input{sections/mechanisms/tables/occupation_results.tex}

        \end{threeparttable}
  \end{table}


Columns (1) and (2) show the estimated effect on native wages of high immigrant concentration occupations. Columns (3) and (4) present the estimated effect on native wages in any occupation with observed immigrants. Columns (5) and (6) show the estimated effect on native wages of occupations with no immigrant presence.

These results suggest that the aggregate market's observed positive effects survive similarly to our economic sector analysis. Specifically, occupations with a high concentration of immigrants experienced on average a 1.3 percent increase in wages. In comparison, occupations with any concentration of immigrants saw a slightly higher increase of 1.7 percent, 1.3 when controlling for covariates. In contrast, occupations with no immigrant presence had the highest wage growth at 3.5 percent, statistically significant at 1 percent.

Combining the last three sets of results gives us a better picture of what happened in Roraima: immigrants arrived, driving general wages up, likely due to labor demand and workers outside formality. However, individuals who could penetrate the formal labor market put downward pressure on native wages. This was not conditional on similar education levels solely, but directly on types of occupations and economic sectors.


==> sections/mechanisms/subsubsections/occupation_mover.tex <==
We can further investigate the substitutability of formal immigrants by examining the job changes of native workers in response to immigration. This is similar to the approach taken in \cite{foged_immigrants_2016}, which assumes that refugees entering the labor market took on manual-intensive jobs, potentially allowing native workers to shift into other occupations. By looking at the degree of job displacement inside the formal labor market, we can better understand whether immigration led to market efficiency changes.

To analyze the effects of immigration on native workers' job choices, we created a binary variable to indicate whether an individual in a high-immigrant occupation ever changed their occupation to a low (or no) immigrant position. We used this variable as the dependent variable in Equation \ref{eq:wagesdid} and present the regression results in Table \ref{tab:occupationmover_results}. They correspond to a linear probability measurement of an individual being a ``mover'' from immigrant occupations to non-immigrant ones, between treatment and control groups.

  \begin{table}[htb!]
   \vspace{1cm}
  \centering 
     \begin{threeparttable}
         \caption{Occupation Mover Analysis} \label{tab:occupationmover_results}
            \input{sections/mechanisms/tables/occupationmover_results.tex}
        \end{threeparttable}
  \end{table}
  
To perform our analysis, we used two versions of the data. The first version includes all observations from the treated and control groups, while the second version is more conservative, only including individuals who consistently worked in non-immigrant occupations during the pre-treatment period. Columns (1) and (2) in the table represent the results for the first data sample, while Columns (3) and (4) represent the results for the second sample.

The values of the first two columns indicate that, overall, there was little net change in job occupations. However, examining the conservative sample shows a significant increase in the probability of changing to a non-immigrant-related job occupation of approximately 13 percent. It is reasonable to assume that the actual effect of immigrants, who have a relatively low representation in the formal labor market on job changes lies around this value.

Moreover, our analysis in Appendix \ref{sec:border_analysis} indicates that the results of our border municipality analysis were inconclusive. Since 90 percent of occupations in the border municipality of Pacaraima involve manual tasks, immigrant workers in formal employment may have substituted for native workers with low skill levels in some sectors, but complemented native workers in other sectors. However, Pacaraima did not have sufficient opportunities in these sectors to benefit from these dynamics.

==> sections/mechanisms/tables/activity_results.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-7}
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{High Immigrant Presence} & \multicolumn{3}{c}{Low Immigrant Presence} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7}
  & (1) & (2) & (3)& (4) & (5) & (6)\\
\midrule
Treated & \num{0.007} & \num{0.004} & \num{0.011} & \num{0.057} & \num{0.061} & \num{0.067}\\
 & (\num{0.009}) & (\num{0.008}) & (\num{0.006}) & (\num{0.018}) & (\num{0.018}) & (\num{0.016})\\
\midrule
Individual FE & X & X & X & X & X & X\\
Year FE & X & X & X & X & X & X\\
Covariates &  & X &  X &  & X & X\\
Balanced Panel Data &  &  & X &  &  & X\\
N & \num{674817} & \num{674817} & \num{283447} & \num{77010} & \num{77010} & \num{42949}\\
\bottomrule
\end{tabular}
\begin{tablenotes}
    \item[1] Standard-errors are clustered by municipality.
    \item[2] Covariates are individual's race, age, age-squared, gender, and education.
\end{tablenotes}


==> sections/mechanisms/tables/educationresults.tex <==

\begin{tabular}[t]{lccccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{9}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-10}
\multicolumn{1}{c}{ } & \multicolumn{9}{c}{Education Level} \\
\cmidrule(l{3pt}r{3pt}){2-10}
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Low Education} & \multicolumn{3}{c}{High School} & \multicolumn{3}{c}{College Degree} \\
\cmidrule(l{3pt}r{3pt}){2-4} \cmidrule(l{3pt}r{3pt}){5-7} \cmidrule(l{3pt}r{3pt}){8-10}
  & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9)\\
\midrule
Treated & \num{0.029} & \num{0.029} & \num{0.050} & \num{0.018} & \num{0.015} & \num{0.027} & \num{0.028} & \num{0.033} & \num{0.033}\\
 & (\num{0.011}) & (\num{0.011}) & (\num{0.011}) & (\num{0.008}) & (\num{0.008}) & (\num{0.007}) & (\num{0.010}) & (\num{0.010}) & (\num{0.010})\\
\midrule
Individual FE & X & X & X & X & X & X & X & X & X\\
Year FE & X & X & X & X & X & X & X & X & X\\
Covariates &  & X & X &  & X & X &  & X & X\\
Balanced Panel Data &  &  & X &  &  & X &  &  & X\\
N & \num{725586} & \num{725586} & \num{139405} & \num{1512687} & \num{1512687} & \num{442464} & \num{230692} & \num{230692} & \num{99664}\\
\bottomrule
\multicolumn{10}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{10}{l}{\rule{0pt}{1em}\textsuperscript{2} Covariates are individual's race, age, age-squared, gender, and education level.}\\
\end{tabular}


==> sections/mechanisms/tables/informal_results.tex <==

\begin{tabular}[t]{lcc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Log Wage in the Informal Labor Market} \\
\cmidrule(l{3pt}r{3pt}){2-3}
  & (1) & (2)\\
\midrule
Treated & \num{-0.243} & \num{-0.235}\\
 & (\num{0.055}) & (\num{0.054})\\
\midrule
N & \num{33855} & \num{33855}\\
Year FE & X & X\\
State FE & X & X\\
Covariates &  & X\\
\bottomrule
\multicolumn{3}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\multicolumn{3}{l}{\rule{0pt}{1em}{\makecell[l]{\textsuperscript{2} Covariates are individual's race, age, \\age-squared, gender, and education level.}}}\\
\end{tabular}


==> sections/mechanisms/tables/occupation_results.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{6}{c}{Log Wage} \\
\cmidrule(l{2pt}r{2pt}r{2pt}){2-7}
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{High Presence} & \multicolumn{2}{c}{Any Presence} & \multicolumn{2}{c}{No Presence} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7}
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treated & \num{0.014} & \num{0.012} & \num{0.017} & \num{0.013} & \num{0.034} & \num{0.039}\\
 & (\num{0.010}) & (\num{0.010}) & (\num{0.009}) & (\num{0.009}) & (\num{0.009}) & (\num{0.009})\\
\midrule

Individual FE & X & X & X & X & X & X\\
Year FE & X & X & X & X & X & X\\
Covariates &  & X &  & X &  & X\\
N & \num{76306} & \num{76306} & \num{1826859} & \num{1826859} & \num{604715} & \num{604715}\\
\bottomrule
\end{tabular}
\begin{tablenotes}
    \item[1] Standard-errors are clustered by municipality.
    \item[2] Covariates are individual's race, age, age-squared, gender, and education.
\end{tablenotes}


==> sections/mechanisms/tables/occupationmover_results.tex <==

\begin{tabular}[t]{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Probability of Moving} \\
\cmidrule(l{3pt}r{3pt}){2-5}
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Unbalanced Sample} & \multicolumn{2}{c}{Balanced Sample} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
  & (1) & (2) & (3) & (4)\\
\midrule
Treated & \num{0.005} & \num{0.004} & \num{0.139} & \num{0.123}\\
 & (\num{0.003}) & (\num{0.002}) & (\num{0.035}) & (\num{0.034})\\
\midrule
Individual FE & X & X & X & X\\
Year FE & X & X & X & X\\
Covariates &  & X &  & X\\
N & \num{1594710} & \num{1594710} & \num{23553} & \num{23553}\\
\bottomrule
\end{tabular}
\begin{tablenotes}
    \item[1] Standard-errors are clustered by municipality.
    \item[2] Covariates are individual's race, age, age-squared, gender, and education level.
    \item[3] Balanced Sample includes only individuals working in immigrant occupations for the entire pre-treatment period.
\end{tablenotes}



==> sections/mechanisms/tables/retention_results.tex <==

\begin{tabular}[t]{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Probability of Job Retention} \\
\cmidrule(l{3pt}r{3pt}){2-5}
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Unbalanced Sample} & \multicolumn{2}{c}{Balanced Sample} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
  & (1) & (2) & (3) & (4)\\
\midrule
Treated & \num{0.001} & \num{0.002} & \num{-0.014} & \num{-0.012}\\
 & (\num{0.040}) & (\num{0.040}) & (\num{0.060}) & (\num{0.060})\\
\midrule
Individual FE & X & X & X & X\\
Year FE & X & X & X & X\\
Covariates &  & X &  & X\\
N & \num{2498772} & \num{2498772} & \num{161259} & \num{161259}\\
\bottomrule
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}{\makecell[l]{\textsuperscript{3} Covariates are individual's race, age, age-squared,\\ gender, and education level.}}}\\

\multicolumn{5}{l}{\rule{0pt}{1em}{\makecell[l]{\textsuperscript{3} Balanced Sample includes only individuals working \\in immigrant occupations for the entire pre-treatment \\period.}}}\\
\end{tabular}


==> sections/mechanisms/tables/sales_results.tex <==

\begin{tabular}[t]{lccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{3}{c}{Sales Index} \\
\cmidrule(l{3pt}r{3pt}){2-4}
\multicolumn{1}{c}{ } & \multicolumn{1}{c}{OLS} & \multicolumn{1}{c}{Continuous} & \multicolumn{1}{c}{Binary} \\

\multicolumn{1}{c}{ } & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Treatment} & \multicolumn{1}{c}{Treatment} \\

\cmidrule(l{3pt}r{3pt}){2-2} \cmidrule(l{3pt}r{3pt}){3-3} \cmidrule(l{3pt}r{3pt}){4-4}
  & (1) & (2) & (3)\\
\midrule
Hundreds of Venezuelans & \num{0.031} & \num{0.027} & \\
 & (\num{0.005}) & (\num{0.009}) & \\
Treat &  &  & \num{0.287}\\
 &  &  & (\num{0.068})\\
\midrule
State FE &  & X & X\\
Month FE &  & X & X\\
N & \num{132} & \num{396} & \num{396}\\
\bottomrule
\multicolumn{4}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\end{tabular}


==> sections/mechanisms/unemployment.tex <==
The mechanisms listed above are based on the assumption that our main results do not suffer from selection bias. It is possible that the sample of native workers is different between pre- and post-treatment periods because of job displacement of Brazilians by the incoming Venezuelans, who are comparatively less educated and willing to accept lower wages. In that case, it would create an upward bias on Brazilian wages.

While RAIS data does not allow us to estimate (un)employment effects since it only captures information on those working in the formal labor market in a particular year, we utilize the RAIS dataset to conduct a series of regressions that examine the impact of the crisis on the displacement of native individuals from their job. Specifically, we construct a binary variable that captures changes in employment status related to dismissals. Individuals who maintain their employment throughout the year are coded as 1, while those who experience a change in status are coded as 0. Essentially, a positive coefficient would suggest that job retention in Roraima is higher on average than in the control states following the crisis, while a negative coefficient would suggest that job displacement is higher in Roraima. The categories of dismissal considered in this analysis include termination by the employer, layoff by the employer, voluntary departure by the employee, transfer, and retirement.

We utilize this binary variable as the outcome in our regression analysis, as outlined in Equation \ref{eq:wagesdid}. This analysis aims to estimate the linear probability of native individuals in Roraima retaining their employment in the wake of the Venezuelan crisis.

\begin{table}[htb]
    \vspace{1cm}
    \centering
    \caption{Employment Retention among Brazilians in Roraima}
    \label{tab:retention_results}
    \resizebox{.6\textwidth}{!}{\input{sections/mechanisms/tables/retention_results.tex}}
\end{table}

Table \ref{tab:retention_results} shows the results of this analysis. Columns (1) and (2), using the sample where we do not account for counterfactuals, show that the probability of job retention (or job displacement, for that matter) for Brazilians was similar between treatment and control groups. In columns (3) and (4), we balance the sample by including individuals who were observed working during the entire pre-treatment period (2007-2013), tracking if they ever changed their status after the crisis. This procedure yields a negative 1.4 percent on average job displacement. However, variations are sufficiently high not to reject the null hypothesis, allowing us to conclude there is no evidence of formal displacements due to the immigration shock.

==> sections/methods/empiricalstrategy.tex <==
To empirically test the effects of Venezuelan immigration on Brazilian wages, we use a panel model with unit and time fixed effects. Our period of interest is from 2007 to 2017, with 2014 as the start of our treatment period. Equation \ref{eq:wagesdid} describes the model:

\begin{equation}
 \label{eq:wagesdid}
    y_{ist} = \beta D_{st} + f(X_{it}) + \theta_u + \alpha_t + \epsilon_{ist}
\end{equation}

Here, $y_{ist}$ is the logarithmic wage of native individual $i$ in a state $s$ and year $t$. $D_{st}$ is the indicator variable that takes the value one if the observation is from Roraima state and the year is after 2013. $\theta_u$ is the unit fixed effects, $\alpha_t$ is the year fixed effect, and $\epsilon_{ist}$ is the error term clustered at the state level. $f(X_{it})$ is a function of covariates allowed to be linear in our model. Covariates are individual characteristics observed in our data: gender, race, age, and education level. Our primary parameter of interest is $\beta$, which explains the average effect of the Venezuelan refugee crisis on wages among the Brazilian citizens in Roraima.

The unit fixed effects, $\theta_u$, either take the form of individual fixed effects, $\theta_i$, or individual-municipality fixed effects, $\theta_{i,m}$, where $m$ is the municipality in RAIS. Specification using individual fixed effects portrays the classic panel fixed effects estimation based on the within-individual variation. Following \cite{foged_immigrants_2016}, the coefficient from the specification using individual-municipality fixed effects, on the other hand, estimates the effects of refugee influx on outcomes of native workers within their municipality spells. Despite the fact we addressed the possibility of immigrants moving around in our identification strategy, natives could be moving to other locations within and outside Roraima after the immigration shock to seek better opportunities, offsetting effects in the long run. If natives remained in place, however, we should not see systematically different estimates between the two approaches.


==> sections/methods/identificationstrategy.tex <==
The geographical setting is crucial for our identification strategy. As shown in Figure \ref{fig:geo_overview}, Venezuela borders the Brazilian states of Amazonas and Roraima, but the Amazon rainforest, mountains, and rivers make it impossible to enter Brazil through Amazonas by land. There are no viable roads, and it would be unreasonable for refugees to undertake such a perilous journey. Venezuelans are permitted to enter Brazil, so they do not need to travel through impassable Amazonas.

Instead, people can enter Brazil from Venezuela through the state of Roraima. The BR-174 highway, represented by the vertical solid line traversing Roraima and Amazonas in Figure \ref{fig:geo_overview}, is the only land transportation route between the two countries, which runs through Roraima starting at the Venezuelan border. This makes Roraima a key transit point in Brazil, but once refugees are in Roraima, they can only practically go as far as Amazonas by land. To reach larger coastal cities, they would need to use air routes. Therefore, Roraima is isolated from the rest of the northern states which leads many refugees to choose to enter and stay there.

This setting provides a natural experiment in which Roraima acts as the treated group. For our control group, we use states that share similar socio-geographical characteristics and are located on the Brazilian border: Acre and Amapá. Acre borders Peru and Bolivia, while Amapá borders Suriname and French Guiana. Like Roraima, these states also have a large portion of their population concentrated in their respective capital cities and are relatively isolated. In particular, Amapá has no inland connection to the rest of Brazil and can only be reached by airplane or boat crossing the Amazon hydrographic basin to reach its capital, Macapá.


\begin{figure}[htb!]%
    \vspace{1cm}
    \centering    
    \caption{Map of Venezuela and Brazil's North Region}%
    \includegraphics[width=0.8\textwidth]{sections/methods/figures/geo_overview.png}
    \label{fig:geo_overview}%
\end{figure}

As per \cite{borjas_how_1997, borjas_labor_2003, borjas_native_2006}, it may be difficult to accurately assess the impacts of immigration on the labor market by considering geography alone due to the potential for spillover effects across regions. However, in our case, Roraima is isolated with high transportation costs, which limits the mobility between states or even within municipalities in the same state. Even so, we address the potential issue of Brazilians moving from Roraima to control states after the refugee crisis, which may bias our estimates. As we explain later, we include an interaction between the individual fixed effects and the corresponding municipality, as proposed by \cite{foged_immigrants_2016} to estimate the effects of within-municipality changes in wages, devoid of the mobility effects of a worker moving away from the treated state due to the crisis.

%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

\subsubsection{Foreign Presence in RAIS}\label{subsubsec:foreign_presence}

\input{sections/methods/presence_venezuelans.tex}

%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\subsubsection{Trends}\label{subsubsec:trends}

%\input{sections/methods/trends.tex}

==> sections/methods/methods.tex <==
\noindent
In this section, we discuss the identification strategy and the empirical strategy used to analyze the labor market impacts of the Venezuelan refugee crisis in Roraima, Brazil. The identification strategy section highlights the geographical setting of the natural experiment, while the empirical strategy section explains the econometric models used to estimate the causal effects.


\subsection{Identification Strategy} \label{subsec:identification_strategy}

\input{sections/methods/identificationstrategy.tex}

%-------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Empirical Strategy}\label{subsec:empirical_strategy}

\input{sections/methods/empiricalstrategy.tex}

==> sections/methods/presence_venezuelans.tex <==
A key assumption of our paper is that refugees were not attracted to high-growth regions, but ended up in Roraima due to its geographical isolation and high transportation costs to move to cities farther from the border. To verify this, we can use the RAIS data to check the location of Venezuelan refugees in our sample. We can also examine wage trends before the crisis to confirm that Roraima’s growth trend was not significantly different from the control regions, which we explore in the following subsection. Figure \ref{fig:venezuelantrend} shows the percentage of Venezuelans in the labor market anually, grouped by treatment and control states. In 2017, Venezuelans represented around 2 percent of Roraima’s formal labor market, while none were observed in Amapá or Acre. Figure \ref{fig:venezuelantrend} supports our assumption by demonstrating that Venezuelans largely remained in Roraima.

\begin{figure}[h!]
\vspace{0.3cm}
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/data/figures/vz_trend.jpeg}  
        \caption{Venezuelans as \% of Labor Market}
        \label{fig:venezuelantrend}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/data/figures/fr_trend.jpeg}  
        \caption{Other Foreigners as \% of Labor Market}
        \label{fig:otherforeignerstrend}
    \end{subfigure}%
    \caption{Proportion of non-Brazilians in the formal labor market for Roraima and the control states}
    \label{fig:foreigntrends}
 \end{figure}

It would be problematic for our experiment setting if any other nationality besides the Venezuelans had a substantial growth in population, either in Roraima or the control states. To ensure that the exponential growth of foreigners we observe is because of the Venezuelan refugees, we create Figure \ref{fig:otherforeignerstrend} by aggregating data on all immigrant nationalities other than Venezuelans and plotting their proportion in the formal labor market. As the figure shows, there is no significant growth in the control states and only negligible growth in Roraima following 2014. The non-zero values we observe for non-Venezuelan immigrant nationalities can be attributed to several factors. First, there is a significant presence of Haitian immigrants in control states due to United Nations peace operations in Haiti that began in the 2000s and remained constant over the study years. Second, there are observations of other Latin American and Bolivian nationals in the data in control states due to the proximity of Acre to Bolivia and the resulting natural population exchange. Finally, some of these foreigners may be Venezuelans with dual citizenship, as they only appeared in Roraima after the crisis began, as Figure \ref{fig:otherforeignerstrend} shows. Since there is no incremental change in these populations in either treatment of control, the non-zero values should not pose a threat to our identification strategy.

Although the RAIS data provides a good overview of Venezuelans entering Brazil and remaining in the state of Roraima, it only includes those in the formal labor market. It could compromise our identification strategy if the control states also had many Venezuelan refugees outside the formal labor market. In Appendix \ref{sec:vz_permanence_in_rr}, we use refugee application data to demonstrate that this is not the case. We show that only Roraima, not the control states, experienced a significant increase in the number of Venezuelan citizens seeking refugee status applications.


==> sections/methods/trends.tex <==
Lastly, we ensure control and treatment groups do not differ in trends before the refugee crisis. Immigrants should be allocating themselves to Roraima due to the geographical closeness and transportation challenges, not to any favorable economic growth that could be happening solely there before the crisis.

Figure \ref{fig:wagetrends} presents the wage trends. Panel \ref{fig:wagetrendsstate} shows the wage trend for treated and control states, while Panel \ref{fig:wagetrendscapital} restricts the sample to their respective capitals. In both figures, we do not see any particular difference in wage trends between the treatment and control groups before the immigration crisis, with a small increase in the gap in later years. Any results driven by our experiments should reveal a positive small if not negligible effect on native wages, which aligns with the literature.

We also provide wage trends restricting the sample to individuals living at the border in Panel \ref{fig:wagetrendsborder}. Since the border municipalities are considerably much smaller than the capital sample, we observe greater variation each year. However, differences across control and treated groups are not necessarily large enough to draw any preliminary conclusion. We should expect negligible effects in the area.

\begin{landscape}
\begin{figure}[h!]
    \centerline{
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/data/figures/state_wagetrends.png}  
        \caption{Wage Trends for the State Market}
        \label{fig:wagetrendsstate}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/data/figures/capital_wagetrends.png}  
        \caption{Wage Trends for the Capital Market}
        \label{fig:wagetrendscapital}
    \end{subfigure} %
        }
    \centerline{
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/data/figures/border_wagetrends.png}  
        \caption{Wage Trends for the Border Market}
        \label{fig:wagetrendsborder}
    \end{subfigure}%
}
    \caption{Wage Trends for Roraima and the Control States}
    \label{fig:wagetrends}
 \end{figure}
\end{landscape}


==> sections/results/results.tex <==
In this section, we present the main results of our paper. In the first set of regressions using Equation \ref{eq:wagesdid}, we explore the immigrants' formal labor market wage effects on Brazilians in the state of Roraima and its capital municipality, Boa Vista.

Table \ref{tab:main_results} reports our coefficient of interest, $\beta$, representing the returns on wages by being in Roraima after the Venezuelan crisis. Column (1) represents our model's result for the state using individual and year fixed effects. On average, Roraima experienced a 3 percent increase in wages after the exodus. Adding the covariate matrix of demographic characteristics in Column (2), there is a negligible decrease in the effect, with its overall magnitude still around the same value as the previous measurement.

Column (3) shows results from the model using individual-municipality fixed effects. If results in Column (3) were different in magnitude or precision from Columns (1) and (2), it would indicate that our geographical isolation assumption was incorrect, given the mobility of Brazilians away from Roraima, and our identification strategy would ultimately generate bias in our measurements. However, Column (3) reveals no distinction between adding the municipality component or leaving it aside, suggesting individuals in our data did not move before and after the shock.

Column (4) uses the same model as Column (2), with the covariate matrix, and individual and year fixed effects. However, we balance the panel data by removing observations with no corresponding time counterfactuals. To balance the RAIS sample, we counted only those Brazilians who appeared in the post-treatment period and worked at least one year before 2014. Any native that worked only in the pre-treatment or the post-treatment was removed. Even with this conservative sample, the result was of similar magnitude at around a 3 percent increase in wages after the crisis compared to the control groups.

\begin{table}[htb!]
\vspace{1cm}
    \centering
    \caption{Venezuelan Immigration Effects on Wage in Roraima and its Capital}
    \label{tab:main_results}
    \resizebox{\textwidth}{!}{\input{sections/results/tables/main_results.tex}}
\end{table}

The first four columns of Table \ref{tab:main_results} represented the states' sample, including all municipalities. But Boa Vista, Roraima's capital, accounts for 90 percent of the labor market. Moreover, it is right on Highway BR-174. As confirmed by the data when we combine Figure \ref{fig:foreigntrends} with Table \ref{Tab:summary_capital}, the vast majority of Venezuelans are located there, also confirmed by journalistic accounts. Accordingly, if we expect the state effects observed in our regressions to be due to the immigration crisis, we should also expect similar results when solely sampling the capitals.

To see this, we redo the analysis using the sample from only the state capitals. Column (5) uses the model with individual and year fixed effects, column (6) adds the covariate matrix, and column (7) uses the balancing framework we used for Column (4). The results are similar to the previous analysis, with a magnitude of around 3 percent.

Our findings indicate that immigrants acted as complements rather than substitutes to the Brazilian formal labor market workers, pushing their wages upwards. We dedicate the remainder of the paper to testing the robustness of these main results and disentangling mechanisms. From now on, we will primarily focus on the capital sample unless stated otherwise.


==> sections/results/tables/main_results.tex <==

\begin{tabular}[t]{lccccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{7}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-8}
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{State} & \multicolumn{3}{c}{State Capital} \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-8}
  & (1) & (2) & (3) & (4) & (5) & (6) & (7)\\
\midrule
Roraima After 2013 & \num{0.031} & \num{0.029} & \num{0.029} & \num{0.030} & \num{0.031} & \num{0.029} & \num{0.030}\\
 & (\num{0.007}) & (\num{0.006}) & (\num{0.006}) & (\num{0.007}) & (\num{0.008}) & (\num{0.007}) & (\num{0.007})\\
\midrule
Individual FE & X & X &  & X & X & X & X\\
Individual x Municipality FE &  &  & X &  &  &  & \\
Year FE & X & X & X & X & X & X & X\\
Covariates &  & X & X & X &  & X & X\\
Balanced Panel Data &  &  &  & X &  &  & X\\
N & \num{1898671} & \num{1898671} & \num{1898671} & \num{1308633} & \num{1581011} & \num{1581011} & \num{1071988}\\
\bottomrule
\multicolumn{8}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\multicolumn{8}{l}{\rule{0pt}{1em}\textsuperscript{2} Covariates are individual's race, age, age-squared, gender, and education level.}\\
\end{tabular}


==> sections/robustnesschecks/eventstudies.tex <==
A key assumption of our study is that in the absence of treatment and conditional on individual controls and individual-year fixed effects, the likelihood of wage changes over time in treated and control states would be identical. While we cannot test the counterfactual in post-treatment years, the pre-treatment trends between the treated and control for the outcome variable should be parallel over time.

To test the assumption of parallel trends, we employ an event study where $\beta$ is disaggregated for every year present in the data. The reference year for comparison is 2013, the year before the treatment started. The estimation strategy is given in Equation \ref{eq:wageses}, where the indicator function $D_{st}$ now takes a separate value for each year within the summation. $\beta_{t}$ explains the average difference between treatment and control groups for that particular year conditional on controls and fixed effects.

 \begin{equation} \label{eq:wageses}
    y_{ist} = \sum^{2017}_{\substack{t = 2007 \\ t \neq 2013}} \beta_{t} D_{st} + f(X_{it}) 
 + \theta_i + \alpha_t + \epsilon_{ist}
\end{equation}

If control and treated groups are comparable before treatment, then $\beta_{t}=0$ for $t \in \{2007, \ldots, 2012\}$. Assuming the only disturbance in Roraima's job market after 2013 is the immigration flow, any variation in the post-treatment period estimates in treatment must be associated with the refugee crisis. We conduct event study analysis at both the state and capital levels. Desirably, effects after 2014 should be positive and slightly increasing.

The event study results for the state and the capital are plotted in Figure \ref{fig:state_mainresults_es} and Figure \ref{fig:capital_mainresults_es} respectively.

\begin{figure}[h!]
\vspace{0.3cm}
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/robustnesschecks/figures/state_mainresults_es.png}  
        \caption{State Event Study}
        \label{fig:state_mainresults_es}
    \end{subfigure}%
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\textwidth]{sections/robustnesschecks/figures/capital_mainresults_es.png}  
        \caption{Capital Event Study}
        \label{fig:capital_mainresults_es}
    \end{subfigure}%
    \caption{Event Study Graphs}
    \label{fig:foreigntrends}
 \end{figure}
 
Both the results related to the state and capital analysis reveal parallel trends in earlier years. They yield pre-treatment estimates not statistically different from zero, with an increasingly upward trend in post-treatment periods. This suggests the difference-in-differences model captured the positive effect of Venezuelans, allowing Brazilians, on aggregate, to increase their wages.

Figure \ref{fig:state_mainresults_es} shows that after the crisis started, natives experienced a 3.6 percent wage increase in 2016 on average and a 5 percent increase in 2017, compared to the control states. As shown in Figure \ref{fig:capital_mainresults_es}, the pattern is similar for the capital municipality. An overwhelming percentage of the population in our study states reside in capital municipalities. Thus, the capital makes up a larger part of the state economy and absorbs most of the economic shock.

The event studies corroborate the argument that immigrants complement the native formal workers. However, several potential channels are driving this effect. First, we do not observe the informal labor market in the RAIS data. Immigrants seeking refugee status potentially work informally while they wait for the bureaucracy to receive a work permit. If our assumption is valid, there would be a significant presence of Venezuelans in the informal market. These individuals will positively affect wages assuming the informal labor market is an imperfect substitute for the formal labor market. The second channel is the Venezuelan in RAIS complementing the native worker occupying jobs in different positions. Also, natives could shift to less manual-intensive jobs and increase their wages. Lastly, as suggested by \cite{bodvarsson_does_2006}, the new population can create a labor demand shock. We devote Section \ref{sec:mechanisms} to disentangle the underlying mechanisms driving these effects.

%allowing natives in this sector to benefit from higher labor demand and therefore, higher wages. We explore these results further in our discussion section on whether this is uniform across all the economic activities with varying refugee presence.

%The construction sector event study in Figure \ref{fig:esconstructioncapital} yielded the most significant results, with 2017 estimate at around 8 percent. While the immigrant presence could create a demand for housing and buildings in general, we believe the Venezuelans do not fully explain these results. According to the IBGE, the northern states of Brazil are notably the ones with the most expensive construction costs, with Roraima being fifth in the 2016 national ranking. By 2017, concrete prices, however, fell for the state, allowing firm owners in the sector to hire more individuals \citep{correa_custo_2018}. Therefore, there is a strong evidence of reverse causality, where immigrants were seeking construction activities as a consequence of higher labor compensation. This is the only sector where we found journalistic evidence of a notable change in input prices. In Appendix \ref{sec:inputprices}, despite data limitation, we provide a small investigation on this concrete price variation. To make sure the positive change in the aggregate market is not entirely driven by the construction sector, we provide in Figure \ref{fig:esnoconstructioncapital} an entire market event study excluding construction. There is a small drop in magnitude for the 2017 estimate, but nevertheless the trend remains the same. 

%Figure \ref{fig:esrestaurantscapital} presents the restaurant sector event study. Confirming our previous model, we do not observe any statistically significant estimates. The 2017 parameter with a positive magnitude of 1.5 percent is is not distinguishable from 2013's. Figure \ref{fig:eshealthcapital} shows the results for the health sector. The increase of 8.8 percent in 2017 barely fails the 5 percent confidence, but it yielded a noticeable positive trend.

%\subsubsection{Border Municipality Event Study}

%Figure \ref{fig:esborder} presents the set of event study regressions for the border municipality of Pacaraima. The smaller sample generated higher variations in the pre-treatment periods, with 2008 and 2009 being problematic when trying to satisfy the parallel trends assumption. 

%If we consider the years after 2009, the assumption holds for Figure \ref{fig:esentiremarketborder}, with a sharp positive variation in 2014, but returning to pre-treatment levels in 2017. Considering the presence of Venezuelans increasing in later years, the result suggests no effect on the aggregate market. 

%A similar pre-treatment pattern is shown in Figure \ref{fig:esretailborder}, the retail sector results. However, there is a sudden decrease in wages in 2015 by around 10 percent, remaining at this level in the next years. In our border sample, as well as in the Brazilian Federal Police report, Venezuelans started immigrating around this time. Moreover, the retail sector is the only sector with a significant presence of Venezuelans in the border labor market, as shown in Table \ref{Tab:summary_border}. To make sure this result is not affected by the problematic years, we provide in column (3) of Table \ref{tab:did_border} a retail market regression without 2008 and 2009. The results remained negative and statistically significant, but now at around 7 percent. 

%The rest of the market in Figure \ref{fig:esnoretailborder} presents an opposite behavior from retail. In 2017, there was a 12 percent increase in wages, with a slightly better parallel trends, suggesting higher labor demand due to individuals crossing the border to consume , but returning to Venezuela  \citep{costa_crise_2016}, and natives in this industry not facing the labor supply shock directly.

%These results indicate the substitution effect was more vigorous in Pacaraima when compared to the capital. As a lean market, Pacaraima could not provide enough opportunities to the natives. They had to accept less advantageous contracts, in comparison to control, in order to remain working in a sector with direct foreign competition. Nevertheless, the rest of the market seemed to have experienced positive wage effects after receiving the immigrants.

%Finally, we need to be careful when drawing any conclusions regarding the border labor market. These variations might be happening due to a smaller sample being used. To address this issue, we provide placebo tests in our discussion section.


==> sections/robustnesschecks/placebo.tex <==
Another concern regarding our findings is whether our results are driven by random effects or some particular effects happening in the control group. We conduct two placebo tests to ensure the estimated parameters are closely related to immigration shocks. The first is using the capital of Rondônia, Vila Velha, as the treatment unit. Rondônia is another bordering state in the Brazilian North region, connected to Bolivia. Results are shown in Table \ref{tab:did_placebo}.

\begin{table}[htb!]
    \vspace{1cm}
        \caption{Placebo Test Results using Rondônia as Treatment}
    \label{tab:did_placebo}
    \centering

    \resizebox{0.66\textwidth}{!}{\input{sections/robustnesschecks/tables/placebo_results.tex}}
\end{table}

We follow the same model framework of our state analysis. Column (1) presents the results using individual and year fixed effects, revealing a negative 0.2 percent change in wages but which is not statistically significant. Adding covariates in Column (2) does not change the outcome, still yielding imprecise values. Column (3) uses the interacted individual-municipality fixed effect. Any variation in results while using this specification could be attributed to Rondônia's higher population density and more connected municipalities. Nevertheless, it still presents negligible results. Lastly, Column (4) uses the balanced panel data, yielding similar results.

Second, we compare individuals from the two control states with one another. If Roraima is the only state affected by the refugee crisis, then there should be no differential effects on wages between the control states. This is what we find in Table \ref{tab:place_between_controls}. The change in wages is neither statistically nor economically significant.

The two placebo tests suggest that the effects observed in our main results are driven by particularities found in Roraima, and not by random effects in the placebo or control groups.

==> sections/robustnesschecks/robustnesschecks.tex <==
In this section, we present the event studies and placebo tests to ensure the robustness of our findings.


\subsection{Event Studies} \label{subsec:eventstudies}
\input{sections/robustnesschecks/eventstudies.tex}

\subsection{Placebo Tests} \label{subsec:placebotests}
\input{sections/robustnesschecks/placebo.tex}




==> sections/robustnesschecks/tables/placebo_results.tex <==
\begin{tabular}[t]{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-5}
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Placebo State Capital} \\
\cmidrule(l{3pt}r{3pt}){2-5}
  & (1) & (2) & (3) & (4)\\
\midrule
Treated & \num{-0.002} & \num{-0.004} & \num{-0.006} & \num{-0.004}\\
 & (\num{0.011}) & (\num{0.010}) & (\num{0.010}) & (\num{0.008})\\
\midrule
Individual FE & X & X &  & X\\
Individual x Municipality FE &  &  & X & \\
Year FE & X & X & X & X\\
Covariates &  & X & X & X\\
Balanced Panel Data &  &  &  & X\\
N & \num{2155167} & \num{2155167} & \num{2155167} & \num{1443895}\\
\bottomrule
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by state.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{2} Covariates are individual's race, age, age-squared, gender, and education level.}\\
\end{tabular}


==> summary_2013.tex <==

\begin{tabular}[t]{lllrr}
\toprule
  &    &     & Control States & Roraima\\
\midrule
 & Age & mean & \num{41.41} & \num{39.70}\\
 & Wage & mean & \num{2560.25} & \num{2998.54}\\
Race & White & Percent & \num{20.43} & \num{27.87}\\
 & Black & Percent & \num{3.04} & \num{2.62}\\
 & Indigenous & Percent & \num{0.19} & \num{0.60}\\
 & Mixed & Percent & \num{58.45} & \num{59.70}\\
 & Not Declared & Percent & \num{17.88} & \num{9.20}\\
Sex & Female & Percent & \num{40.61} & \num{36.74}\\
 & Male & Percent & \num{59.39} & \num{63.26}\\
Education & No High School & Percent & \num{34.90} & \num{25.97}\\
 & High School & Percent & \num{47.80} & \num{55.57}\\
 & College & Percent & \num{17.30} & \num{18.46}\\
 & All & N & \num{11413.00} & \num{3315.00}\\
\bottomrule
\end{tabular}


==> summary_2018.tex <==

\begin{tabular}[t]{lllrr}
\toprule
  &    &     & Brazilian & Venezuelan\\
\midrule
 & Age & mean & \num{36.86} & \num{31.67}\\
 & Wage & mean & \num{2857.94} & \num{1198.41}\\
Race & White & Percent & \num{6.18} & \num{5.85}\\
 & Black & Percent & \num{1.07} & \num{1.76}\\
 & Indigenous & Percent & \num{0.33} & \num{0.03}\\
 & Mixed & Percent & \num{34.04} & \num{52.94}\\
 & Not Declared & Percent & \num{58.38} & \num{39.43}\\
Sex & Female & Percent & \num{48.68} & \num{23.96}\\
 & Male & Percent & \num{51.32} & \num{76.04}\\
Education & No High School & Percent & \num{16.97} & \num{16.29}\\
 & High School & Percent & \num{54.97} & \num{76.01}\\
 & College & Percent & \num{28.05} & \num{7.69}\\
 & All & N & \num{128389} & \num{3523}\\
\bottomrule
\end{tabular}


==> tab2_immiact.tex <==

\begin{tabular}[t]{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Log Wage} & \multicolumn{2}{c}{Job Retainment} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
  & (1) & (2) & (3) & (4)\\
\midrule
Treat: Binary & \num{0.019}*** &  & \num{0.023}*** & \\
 & (\num{0.005}) &  & (\num{0.007}) & \\
Treat: VZ Ratio x 100 &  & \num{0.019}*** &  & \num{0.014}**\\
 &  & (\num{0.002}) &  & (\num{0.005})\\
\midrule
Individual FE & X & X & X & X\\
Year FE & X & X & X & X\\
R2 & \num{0.871} & \num{0.872} & \num{0.940} & \num{0.940}\\
R2 Adj. & \num{0.855} & \num{0.855} & \num{0.931} & \num{0.931}\\
RMSE & \num{0.241} & \num{0.241} & \num{0.200} & \num{0.200}\\
N Clusters & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000}\\
N & \num{534212} & \num{534212} & \num{34093} & \num{34093}\\
\bottomrule
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{2} Propensity score explanatory variables are gender and race indicators, age, age-squared, tenure, tenure-squared and education level.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{3} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab2_immiocc.tex <==

\begin{tabular}[t]{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-3}
  & (1) & (2) & (3) & (4)\\
\midrule
Treat: Binary & \num{0.022}*** &  & \num{0.027}*** & \\
 & (\num{0.005}) &  & (\num{0.009}) & \\
Treat: VZ Ratio x 100 &  & \num{0.021}*** &  & \num{0.030}***\\
 &  & (\num{0.003}) &  & (\num{0.005})\\
\midrule
Individual FE & X & X & X & X\\
Year FE & X & X & X & X\\
R2 & \num{0.884} & \num{0.885} & \num{0.963} & \num{0.963}\\
R2 Adj. & \num{0.870} & \num{0.870} & \num{0.953} & \num{0.953}\\
RMSE & \num{0.244} & \num{0.243} & \num{0.183} & \num{0.183}\\
N Clusters & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000}\\
N & \num{551954} & \num{551954} & \num{22651} & \num{22651}\\
\bottomrule
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{2} Propensity score explanatory variables are gender and race indicators, age, age-squared, tenure, tenure-squared and education level.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{3} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_education.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-3}
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat: Binary & \num{-0.037}*** &  & \num{0.015}*** &  & \num{0.041}*** & \\
 & (\num{0.006}) &  & (\num{0.004}) &  & (\num{0.012}) & \\
Treat: VZ Ratio x 100 &  & \num{-0.013}*** &  & \num{0.017}*** &  & \num{0.042}***\\
 &  & (\num{0.003}) &  & (\num{0.003}) &  & (\num{0.007})\\
\midrule
Individual FE & X & X & X & X & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.905} & \num{0.905} & \num{0.867} & \num{0.868} & \num{0.883} & \num{0.883}\\
R2 Adj. & \num{0.886} & \num{0.886} & \num{0.845} & \num{0.845} & \num{0.857} & \num{0.857}\\
RMSE & \num{0.272} & \num{0.272} & \num{0.236} & \num{0.236} & \num{0.181} & \num{0.181}\\
N Clusters & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000}\\
N & \num{60575} & \num{60575} & \num{335147} & \num{335147} & \num{176071} & \num{176071}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} Propensity score explanatory variables are gender and race indicators, age, age-squared, tenure, tenure-squared and education level.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{3} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_immimover.tex <==

\begin{tabular}[t]{lcc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Log Wage} & \multicolumn{2}{c}{Job Retainment} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
  & (1) & (2)\\
\midrule
Treat: Binary & \num{0.002}*** & \\
 & (\num{0.000}) & \\
Treat: VZ Ratio x 100 &  & \num{0.001}***\\
 &  & (\num{0.000})\\
\midrule
Individual FE & X & X\\
Year FE & X & X\\
R2 & \num{0.118} & \num{0.118}\\
R2 Adj. & \num{0.008} & \num{0.008}\\
RMSE & \num{0.072} & \num{0.072}\\
N Clusters & \num{53.000} & \num{53.000}\\
N & \num{576800} & \num{576800}\\
\bottomrule
\multicolumn{3}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{3}{l}{\rule{0pt}{1em}\textsuperscript{2} Propensity score explanatory variables are gender and race indicators, age, age-squared, tenure, tenure-squared and education level.}\\
\multicolumn{3}{l}{\rule{0pt}{1em}\textsuperscript{3} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_immiocc.tex <==

\begin{tabular}[t]{lcccccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Log Wage} \\
\cmidrule(l{3pt}r{3pt}){2-3}
  & (1) & (2) & (3) & (4) & (5) & (6)\\
\midrule
Treat: Binary & \num{0.005} &  & \num{0.025}*** &  & \num{0.064}*** & \\
 & (\num{0.005}) &  & (\num{0.008}) &  & (\num{0.015}) & \\
Treat: VZ Ratio x 100 &  & \num{0.012}*** &  & \num{0.025}*** &  & \num{0.043}***\\
 &  & (\num{0.002}) &  & (\num{0.005}) &  & (\num{0.008})\\
\midrule
Individual FE & X & X & X & X & X & X\\
Year FE & X & X & X & X & X & X\\
R2 & \num{0.885} & \num{0.885} & \num{0.963} & \num{0.963} & \num{0.872} & \num{0.873}\\
R2 Adj. & \num{0.867} & \num{0.867} & \num{0.952} & \num{0.952} & \num{0.846} & \num{0.846}\\
RMSE & \num{0.253} & \num{0.253} & \num{0.183} & \num{0.183} & \num{0.169} & \num{0.169}\\
N Clusters & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000}\\
N & \num{382836} & \num{382836} & \num{22851} & \num{22851} & \num{168918} & \num{168918}\\
\bottomrule
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{2} Propensity score explanatory variables are gender and race indicators, age, age-squared, tenure, tenure-squared and education level.}\\
\multicolumn{7}{l}{\rule{0pt}{1em}\textsuperscript{3} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_main.tex <==

\begin{tabular}[t]{lcccc}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Log Wage} & \multicolumn{2}{c}{Job Retainment} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5}
  & (1) & (2) & (3) & (4)\\
\midrule
Treat: Binary & \num{0.022}*** &  & \num{-0.010} & \\
 & (\num{0.006}) &  & (\num{0.010}) & \\
Treat: VZ Ratio x 100 &  & \num{0.021}*** &  & \num{0.001}\\
 &  & (\num{0.003}) &  & (\num{0.005})\\
\midrule
Individual FE & X & X & X & X\\
Year FE & X & X & X & X\\
R2 & \num{0.888} & \num{0.889} & \num{0.244} & \num{0.244}\\
R2 Adj. & \num{0.875} & \num{0.875} & \num{0.150} & \num{0.150}\\
RMSE & \num{0.245} & \num{0.245} & \num{0.370} & \num{0.370}\\
N Clusters & \num{53.000} & \num{53.000} & \num{53.000} & \num{53.000}\\
N & \num{577552} & \num{577552} & \num{577552} & \num{577552}\\
\bottomrule
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{1} Standard-errors are clustered by municipality.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{2} Propensity score explanatory variables are gender and race indicators, age, age-squared, tenure, tenure-squared and education level.}\\
\multicolumn{5}{l}{\rule{0pt}{1em}\textsuperscript{3} * p < 0.1, ** p < 0.05, *** p < 0.01}\\
\end{tabular}


==> tab_summary_2013.tex <==

\begin{tabular}[t]{lllrr}
\toprule
  &    &     & Control States & Roraima\\
\midrule
 & Age & mean & \num{41.41} & \num{39.70}\\
Sex & Female & Percent & \num{40.61} & \num{36.74}\\
 & Male & Percent & \num{59.39} & \num{63.26}\\
Race & White & Percent & \num{20.43} & \num{27.87}\\
 & Black & Percent & \num{3.04} & \num{2.62}\\
 & Indigenous & Percent & \num{0.19} & \num{0.60}\\
 & Mixed & Percent & \num{58.45} & \num{59.70}\\
 & Not Declared & Percent & \num{17.88} & \num{9.20}\\
Education & No High School & Percent & \num{34.90} & \num{25.97}\\
 & High School & Percent & \num{47.80} & \num{55.57}\\
 & College & Percent & \num{17.30} & \num{18.46}\\
 & All & N & \num{11413.00} & \num{3315.00}\\
\bottomrule
\end{tabular}


==> tab_summary_2018.tex <==

\begin{tabular}[t]{lllrr}
\toprule
  &    &     & Brazilian & Venezuelan\\
\midrule
 & Age & mean & \num{36.86} & \num{31.67}\\
Race & White & Percent & \num{6.18} & \num{5.85}\\
 & Black & Percent & \num{1.07} & \num{1.76}\\
 & Indigenous & Percent & \num{0.33} & \num{0.03}\\
 & Mixed & Percent & \num{34.04} & \num{52.94}\\
 & Not Declared & Percent & \num{58.38} & \num{39.43}\\
Sex & Female & Percent & \num{48.68} & \num{23.96}\\
 & Male & Percent & \num{51.32} & \num{76.04}\\
Education & No High School & Percent & \num{16.97} & \num{16.29}\\
 & High School & Percent & \num{54.97} & \num{76.01}\\
 & College & Percent & \num{28.05} & \num{7.69}\\
 & All & N & \num{128389} & \num{3523}\\
\bottomrule
\end{tabular}

